Recon: Reducing Conflicting Gradients from the Root for Multi-Task Learning

A fundamental challenge for multi-task learning is that different tasks may conflict with each other when they are solved jointly, and a cause of this phenomenon is conflicting gradients during optimization. Recent works attempt to mitigate the influence of conflicting gradients by directly altering the gradients based on some criteria. However, our empirical study shows that ``gradient surgery'' cannot effectively reduce the occurrence of conflicting gradients. In this paper, we take a different approach to reduce conflicting gradients from the root. In essence, we investigate the task gradients w.r.t. each shared network layer, select the layers with high conflict scores, and turn them to task-specific layers. Our experiments show that such a simple approach can greatly reduce the occurrence of conflicting gradients in the remaining shared layers and achieve better performance, with only a slight increase in model parameters in many cases. Our approach can be easily applied to improve various state-of-the-art methods including gradient manipulation methods and branched architecture search methods. Given a network architecture (e.g., ResNet18), it only needs to search for the conflict layers once, and the network can be modified to be used with different methods on the same or even different datasets to gain performance improvement. The source code is available at https://github.com/moukamisama/Recon.

==> Fig/Fig_Ablation_Hyperparameters.tex <==
\begin{figure}[!htbp]
    \centering
  \includegraphics[width=0.3\linewidth]{example-image}
  \caption{Study of hyperparameters on MultiFashion+MNIST benchmark. (a) The ablation study on the conflict severity $L$. (b) The ablation study on of selected layers $K$.}
  \label{fig:ablation_hyperparameter}
\end{figure}

==> Fig/Fig_Ablation_K.tex <==
\begin{figure}[!tbp]
    \centering
\subfigure[]{
\includegraphics[width=0.26\textwidth]{Fig/Ablation_K.pdf}
}
\subfigure[]{
\includegraphics[width=0.26\textwidth]{Fig/Ablation_S.pdf}
}
\caption{The performance of CAGrad combined with Recon on the Multi-Fashion+MNIST benchmark with (a) different number of selected layers $K$ (b) different severity value $S$ for computing conflict scores.}   \label{fig:hyperparameters}
\end{figure}

==> Fig/Fig_Ablation_S.tex <==
\begin{figure}[!tbp]
    \centering

\includegraphics[width=0.99\linewidth]{Fig/Ablation_S.pdf}
  \caption{xx}

  \label{fig: xx}
\end{figure}

==> Fig/Fig_Method_Illustration.tex <==
\begin{figure}[H]
    \centering
  \includegraphics[width=0.65\linewidth]{Fig/approach_illustration.pdf}
  \caption{\textcolor{blue}{
  Turning the shared layers with high conflict scores to task-specific layers.
  %The illustration of Recon. First, we compute $S$-conflict scores for each shared layer. Next, we set the layers with high conflict scores to be task-specific and train the modified network from scratch.
  }}
  \label{fig:approach_illustration}
\end{figure}
